A New Upper Bound on Cache Hit Probability for Non-anticipative Caching Policies

Caching systems have long been crucial for improving the performance of a wide variety of network and web based online applications. In such systems, end-to-end application performance heavily depends on the fraction of objects transferred from the cache, also known as the cache hit probability. Many caching policies have been proposed and implemented to improve the hit probability. In this work, we propose a new method to compute an upper bound on hit probability for all non-anticipative caching policies, i.e., for policies that have no knowledge of future requests. Our key insight is to order the objects according to the ratio of their Hazard Rate (HR) function values to their sizes and place in the cache the objects with the largest ratios till the cache capacity is exhausted. Under some statistical assumptions, we prove that our proposed HR to size ratio based ordering model computes the maximum achievable hit probability and serves as an upper bound for all non-anticipative caching policies. We derive closed form expressions for the upper bound under some specific object request arrival processes. We also provide simulation results to validate its correctness and to compare it to the state-of-the-art upper bounds. We find it to be tighter than state-of-the-art upper bounds for a variety of object request arrival processes.

==> hr-policy.tex <==
%%!TEX PS-program = pdflatexmk
%!TEX root = HR_bound_ToMPECS.tex
Our upper bound will be obtained for the  so-called {\em hazard rate} policy for equal\footnote{The content sizes are assumed to be equal to $1.$ If not equal to $1$, then we assume $B$ to be an integral multiple of the content size.} sized contents, abbreviated as HR-E.  Any time $t$, HR-E determines the hazard rate function of all contents. To determine these $n$ quantities, let $\tau_i(t)$ be the last time before $t$ where content $i$ was requested. The hazard rate function of content $i$ at time $t$ is given by 
\[
\Lambda_i(t):=\lambda^*_i(t-\tau_i(t)).
\]
Thus we define the following HR based policy.\\

\noindent{\bf HR-E:} 
{\it
At time $t$, HR-E places in the cache the $B$ contents which have the largest  hazard rate functions, {\em i.e.} if 
$\Lambda_{i_1}(t)>\cdots>\Lambda_{i_n}(t)$ then contents $i_1,\ldots,i_B$ are cached at time $t$. \\
}

Below, we state and prove a lemma and a theorem that show the hit probability under HR-E is an upper bound on the cache hit probability for all on-demand online  caching policies ({\em i.e.} all policies in $\Pi$).

%\footnote{We call HR-E policy as HR for brevity.} 
\begin{lemma}\label{lemma:1}
For $K\geq 1$, 
\begin{align}
\label{lem:res}
\mathbb{E}[N_K^{HR-E}] \ge \mathbb{E}[N_K^{\pi}], \quad \forall \pi \in \Pi.
\end{align}
\end{lemma}
\begin{proof}
Let $\pi\in \Pi$. Given a request arrives at time $t$, it is for content $i$ with the probability 
\begin{align}\label{eq:prob}
p_i(t):=\Lambda_i(t)/\sum_{j=1}^n \Lambda_j(t),
\end{align}
\noindent Note that, $p_i(t)$ is independent of $\pi$. Hence, for any $k$,
\begin{eqnarray}
P(R_k\in B^\pi_k)&=& \frac{\sum_{i\in B_{k}^{\pi}} \Lambda_i(T_k)}{ \sum_{j=1}^n \Lambda_j(T_k)}\nonumber\\
&\leq & \frac{\sum_{i\in B_{k}^{HR-E}} \Lambda_i(T_k)}{ \sum_{j=1}^n \Lambda_j(T_k)}\label{lem:inq}\\
&=&\Prob(R_k\in B^{HR-E}_k),
\label{lem-inq2}
\end{eqnarray}
%\begin{eqnarray}
%P(R_k\in B^\pi_k)&=& \frac{\sum_{i\in B_{k}^{\pi}} \Lambda_i(T_k)}{ \sum_{j\in B_{k}^{\pi}} \Lambda_j(T_k)}\nonumber\\
%&\geq & \frac{\sum_{i\in B_{k}^{HR}} \Lambda_i(T_k)}{ \sum_{j\in B_{k}^{HR}} \Lambda_j(T_k)}\label{lem:inq}\\
%&=&\Prob(R_1\in B^{HR}_k),
%\label{lem-inq2}
%\end{eqnarray}
where (\ref{lem:inq}) follows from the definition of policy HR-E, which at any time caches the $B$ contents with the highest hazard rate functions at this time. Summing both sides of (\ref{lem-inq2}) for $k=0,\ldots,K-1$ yields (\ref{lem:res}) from the very definition of $\E[N^\pi_K]$.
\end{proof}
%
%Lemma \ref{lem:res} actually holds under the only assumption that  each content request process forms a regular point process on $[0,\infty)$ \cite{} 
%({\em i.e.} the inter-request times for a  given content do not need to be a stationary and ergodic process, and these $n$ processes do not need to be independent). More specifically, let $0\leq T_{i,0}<T_{i,1}<\cdots$ be the successive time instants where content 
%$i=1,\ldots,n$ is requested,  and let $\lambda^*_{i,k}(t)$ be the hazard rate function of $X_{i,k}:=T_{i,k}-T_{i,k-1}$ (by convention $T_{i,-1}=0$). It is given by
%\[
%\lambda^*_{i,k}(t)=\left\{\begin{array}{ll}
% \frac{f_{i,1}(t)}{1-F_{i,1}(t)}&\mbox{for $t>0,k=0$}\\
%  \frac{f_{i,k}(t; t_{i,1}, \ldots, t_{i,k-1})}{1-F_{i,k}(t; t_{i,j}, t_{i,1}, \ldots, t_{i,k-1})}&\mbox{for $t> t_{i,k-1}, k\geq 1$},
% \end{array}
%\right.
%\]
%$F_{i,k}(t; t_{i,1}, \ldots, t_{i,k-1}) =\Prob(X_{i,k}<t-T_{i,k-1}\,|\,T_{i,j}=t_{i,j}, 1\leq j\leq k-1)$ and $f_{i,k}(t; t_{i,1}, \ldots, t_{i,k-1}))=\frac{d}{dt}F_{i,k}(t; t_{i,1}, \ldots, t_{i,k-1})$
%(the latter derivative exists when the point process $\{T_{i,k},k\in\N\}$ is regular \cite[Prop. 7.2.IV]{Daley2003}).
%Let $B^\pi_0$ (resp. $B^{HR-E}_0$) be the content of the cache under $pi$ (resp. HR) at time $t=0$. Then, the proof of Lemma \ref{lem:res}  holds
%for any value of $B^\pi_0$ and $B^{HR-E}_0$ if $\Lambda_i(t)$ is replaced by $\lambda^*_{i,k}(t-\tau_i(t))$.
%
%
\begin{theorem}
$h^{HR-E} \ge \max\limits_{\pi \in \Pi} h^{\pi}$.
\end{theorem}
\begin{proof}
Follows from \eqref{def-h2} and Lemma \ref{lemma:1}.
\end{proof}

\begin{remark}
Note that, the HR-E policy does not require keeping track of usage information of the contents. Thus it is easy to simulate and implementable when prefetching overheads are negligible.
\end{remark}

\begin{remark}
Also, note that to compute HR-E based upper bound one does not need to implement HR-E policy.  For each arrival of content $R_k$ at time $T_k$, one can evaluate the HR function values at time $T_k$ for all contents. One can then treat the request $R_k$ as a hit if the hazard rate of $R_k$ is among the top $B$ hazard rates at time $T_k$.
\end{remark}
%\begin{theorem}
%$h^{HR} \ge \max\limits_{\pi \in \Pi} h^{\pi}$.
%\end{theorem}
%\begin{proof}
%Let $\pi\in \Pi$. Given a request arrives at time $t$, it is for content $i$ with the probability 
%$$p_i(t):= \frac{\Lambda_i(t)}{\sum\limits_{j=1}^n \Lambda_j(t)},$$ 
%Note that, $p_i(t)$ is independent of $\pi$. Recall the definitions of $B^\pi_k$ and $N_K^{\pi}$ given in the previous section.  For any $k$,
%\begin{eqnarray}
%P(R_k\in B^\pi_k)&=& \frac{\sum_{i\in B_{k}^{\pi}} \Lambda_i(T_k)}{ \sum_{j=1}^n \Lambda_j(T_k)}\nonumber\\
%&\leq & \frac{\sum_{i\in B_{k}^{HR}} \Lambda_i(T_k)}{ \sum_{j=1}^n \Lambda_j(T_k)}\label{lem:inq}\\
%&=&\Prob(R_k\in B^{HR}_k),
%\label{lem-inq2}
%\end{eqnarray}
%%\begin{eqnarray}
%%P(R_k\in B^\pi_k)&=& \frac{\sum_{i\in B_{k}^{\pi}} \Lambda_i(T_k)}{ \sum_{j\in B_{k}^{\pi}} \Lambda_j(T_k)}\nonumber\\
%%&\geq & \frac{\sum_{i\in B_{k}^{HR}} \Lambda_i(T_k)}{ \sum_{j\in B_{k}^{HR}} \Lambda_j(T_k)}\label{lem:inq}\\
%%&=&\Prob(R_1\in B^{HR}_k),
%%\label{lem-inq2}
%%\end{eqnarray}
%where (\ref{lem:inq}) follows from the definition of policy $HR$, which at any time caches the $B$ contents with the highest hazard rate functions at this time. From the very definition of $\E[N^\pi_K]$, summing both sides of (\ref{lem-inq2}) for $k=0,\ldots,K-1$ yields
%\begin{align}
%\label{lem:res}
%\mathbb{E}[N_K^{HR}] \ge \mathbb{E}[N_K^{\pi}], \quad \forall \pi \in \Pi, \quad K\ge 1.
%\end{align}
%It follows from (\ref{def-h2}) and Equation \eqref{lem:res} that 
%$$h^{HR} \ge \max\limits_{\pi \in \Pi} h^{\pi}$$.
%\end{proof}

%\begin{align}
%&\mathbb{P}(R_k \in B_{t}^{HR}) = \sum\limits_{j=1}^{n} \mathbb{P}(R_k = j) \mathbb{P}(j \in B_{t}^{HR})  \nonumber\\&=  \sum\limits_{j=1}^{n} \mathbb{P}(R_k = j) \frac{\sum\limits_{i=1}^B \lambda^*_{[i]}(t)}{\sum\limits_{j=1}^n \lambda^*_{j}(t)}.
%\end{align}

%\noindent {\bf Question 1:} Is it true that $\mathbb{P}(R_k = j) \propto  \lambda^*_{j}(t)?$\\
%
%\noindent {\bf Question 2:} Is it true that $\mathbb{P}(j \in B_{t}^{HR}) \propto   \frac{\sum\limits_{i=1}^B \lambda^*_{[i]}(t)}{\sum\limits_{j=1}^n \lambda^*_{j}(t)}?$\\
%
%\noindent {\bf Question 3:} How to get an upper bound on  $\mathbb{P}(j \in B_{t}^{\pi})$, {\em i.e.} how to prove $\mathbb{P}(j \in B_{t}^{\pi}) \le \mathbb{P}(j \in B_{t}^{HR})?$

%\subsection{Extension to non-stationary processes}
%Our HR bound applies to any content request process which can be associated with a hazard rate at all values of time $t$. For example, consider the following non-stationary request processes. 
%
%{\it Let the request arrival process for content $i$ is described by a non-homogeneous Poisson process having intensity function $\lambda(t)$. Let the last request for the content arrived at time $x$. Then the hazard rate function at time $t>x$ is given by $\lambda(x+t)$. Thus the hazard rate function is well defined for some of the non-stationary request processes and hence our HR bound.}
